Amortized variance reduction for doubly stochastic objectives

Approximate inference in complex probabilistic models such as deep Gaussian processes requires the optimisation of doubly stochastic objective functions. These objectives incorporate randomness both from mini-batch subsampling of the data and from Monte Carlo estimation of expectations. If the gradient variance is high, the stochastic optimisation problem becomes difficult with a slow rate of convergence. Control variates can be used to reduce the variance, but past approaches do not take into account how mini-batch stochasticity affects sampling stochasticity, resulting in sub-optimal variance reduction. We propose a new approach in which we use a recognition network to cheaply approximate the optimal control variate for each mini-batch, with no additional model gradient computations. We illustrate the properties of this proposal and test its performance on logistic regression and deep Gaussian processes.

==> sections/theoretical.tex <==
\section{THEORETICAL ANALYSIS}

We introduced control variates to reduce the gradient variance and thereby improve the optimisation behaviour. In this section we show how controlling the gradient can improve the convergence behaviour of Stochastic Gradient Descent (SGD), in an ideal situation.

Consider the function $f(\vepsilon,\params): \R^D\times \R^P \rightarrow \R$, where $\vepsilon$ is a random variable distributed according to $p(\vepsilon)$. 
We want to solve the following optimisation problem using SGD,
\begin{equation}
    \myeqnstyle
    \min_{\params} \E_{p(\vepsilon)}[f(\vepsilon,\params)].
\end{equation}
We assume $\E_{p(\vepsilon)}[f(\vepsilon, \params)]$ is strongly convex and smooth as defined below.  
SGD starts with an initial guess for the optimal parameter $\params_0$. The parameter is then sequentially updated according to
\begin{equation}
\params_{t+1} = \params_{t} - \eta_{t}\hat{\vg}(\vepsilon_t,\params_{t}),
\end{equation}
where $\vepsilon_t$ is an independent realisation (over $t$)  of $\vepsilon$ at time $t$, $\hat{\vg}(\vepsilon_t, \params_t) = \nabla_{\params} f(\vepsilon_t, \params_t)$, and $\eta_t\in \R$ is a constant.
We want to reduce the variance in the update direction by setting 
\begin{equation}
\label{eqn:control_term}
\tilde{\vg}(\vepsilon,\params) = \hat{\vg}(\vepsilon,\params) - \vc(\vepsilon,\params),
\end{equation}
where $\vc(\vepsilon,\params): \R^D \times \R^P \rightarrow \R^P$ is a control term designed to reduce the randomness in $\hat{\vg}(\vepsilon, \params)$. This gives a new update rule
\begin{equation}
    \label{eqn:cv_update_rule}
    \params_{t+1} = \params_{t} - \eta_{t}\tilde{\vg}(\vepsilon_t,\params_t) .
\end{equation}
We can show that adding a control term as in \cref{eqn:control_term} yields a better convergence rate for SGD under the following assumptions:
\begin{assumption}[Smoothness]
\label{thm:assumption_1}
$f(\vepsilon,\params)$ is $L$ smooth in $\params$ (for some $L>0$), i.e.
\begin{equation*}
f(\vepsilon,\params')- f(\vepsilon,\params) \le (\params'-\params)\transpose \nabla f(\vepsilon,\params) + \frac{1}{2}L\|\params'-\params\|_2^2,
\end{equation*}
\end{assumption}

\begin{assumption}[Strong Convexity]
\label{thm:assumption_2}
$f(\vepsilon, \params)$ is $H$ strongly convex in $\params$ (for some $H>0$), i.e.
\begin{gather*}
f(\vepsilon,\params')- f(\vepsilon,\params) \ge (\params'-\params)\transpose\nabla f(\vepsilon,\params)  + \frac{1}{2}H\|\params'-\params\|_2^2,
\end{gather*}
\end{assumption}

\begin{assumption}[Efficient Control Variate] The norm of the controlled gradient is bounded by a constant $M$ as
\label{thm:assumption_3}
\begin{equation*}
\E \big[\|\nabla f(\vepsilon,\params^*) - c(\vepsilon,\params)\|_2^2 \big] \le M\E [f(\vepsilon,\params) - f(\vepsilon,\params^*)].
\end{equation*}
\end{assumption}

\begin{theorem}[Convergence Rate]\label{T:Convergence}
Under assumptions \ref{thm:assumption_1}, \ref{thm:assumption_2} and \ref{thm:assumption_3}, with $\eta_t=\eta\le\frac{1}{2L+M}$ for all $t$, the update rule given by \cref{eqn:cv_update_rule} offers a linear convergence rate. Specifically, there exists $0<c<1$ (depending on $H$, $L$ and $M$ as specified in \cref{appx:appendix_a}) such that
\begin{equation}
\E\bigg[ \|\params_t-\params^*\|_2^2\bigg] \le c^t
\|\params_0-\params^*\|_2^2.
\end{equation}
\end{theorem}

\begin{proof}
See \cref{appx:appendix_a}.
\end{proof}

Although the above assumptions do not necessarily hold in practice, 
Theorem~\ref{T:Convergence} is useful in giving intuition into the convergence speed of our proposed method. This theorem gives a sufficient condition for the control variate which guarantees the fast convergence rate similar to that of (non-stochastic) gradient descent and stochastic variance reduced gradient descent (SVRG) \citep{Johnson2013svrg}. Specifically, if Assumption 3 holds, our method offers the so called linear convergence rate.

We can relax Assumption 3 as the following assumption. 
\begin{assumption} The norm of the controlled gradient is bounded as
\label{thm:assumption_4}
\begin{equation*}
\E \big[\|\nabla f(\vepsilon,\params^*) - c(\vepsilon,\params)\|_2^2 \big] \le \bar{M}.
\end{equation*}
\end{assumption}

Under assumptions \ref{thm:assumption_1}, \ref{thm:assumption_2} and \ref{thm:assumption_4}, with $\eta_t=\eta\le\frac{1}{2L}$ for all $t$, for the update rule given by \cref{eqn:cv_update_rule}, there exists $0<\bar{c}<1$ (depending on $H$ and $L$ as specified in \cref{appx:appendix_a}) such that
\begin{equation}\label{eqn:convass4}
\E\bigg[ \|\params_t-\params^*\|_2^2\bigg] \le \bar{c}^t
\|\params_0-\params^*\|_2^2  +\frac{2\eta^2\bar{M}(1 - \bar{c}^t)}{1 - \bar{c}}.
\end{equation}
This result shows that the more efficient the control variate (the smaller $\bar{M}$), the smaller the error in optimisation ($||\params_t-\params^*||_2^2$). For the detail on the proof of~\eqref{eqn:convass4} see \cref{appx:appendix_a}.


%\ticomment{TODO: We can relax assumption 3, only assuming a constant upper bound on the quality of the control variate (instead of a decreasing upper bound as so far). This will affect the convergence rate though. With the new assumption we can prove a sublinear convergence rate (similar to SGD) rather than a linear one (the current result). Add in Appendix, mention here.}

